Why flatness does and does not correlate with generalization for deep neural networks

The intuition that local flatness of the loss landscape is correlated with better generalization for deep neural networks (DNNs) has been explored for decades, spawning many different flatness measures. Recently, this link with generalization has been called into question by a demonstration that many measures of flatness are vulnerable to parameter re-scaling which arbitrarily changes their value without changing neural network outputs. Here we show that, in addition, some popular variants of SGD such as Adam and Entropy-SGD, can also break the flatness-generalization correlation. As an alternative to flatness measures, we use a function based picture and propose using the log of Bayesian prior upon initialization, $\log P(f)$, as a predictor of the generalization when a DNN converges on function $f$ after training to zero error. The prior is directly proportional to the Bayesian posterior for functions that give zero error on a test set. For the case of image classification, we show that $\log P(f)$ is a significantly more robust predictor of generalization than flatness measures are. Whilst local flatness measures fail under parameter re-scaling, the prior/posterior, which is global quantity, remains invariant under re-scaling. Moreover, the correlation with generalization as a function of data complexity remains good for different variants of SGD.

==> bin.tex <==
\iffalse
\begin{figure*}[h!]
\centering
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-sensitivity_logits-generalization.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-sensitivity_sigmoid-generalization.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-robustness_logits-generalization.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-robustness_sigmoid-generalization.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-sensitivity_logits-generalization-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-sensitivity_sigmoid-generalization-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-robustness_logits-generalization-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/MNIST-robustness_sigmoid-generalization-on-test.png}}

\caption{The correlation between input sensitivity, robustness and generalization on MNIST, $|S|=500, |E|=1000$. The optimizer is vanilla SGD. Architecture: FCN.
Here "logits" means the we use the output before the final activation (softmax or sigmoid in binary dataset).
(a)-(d): The metrics (sensitivity and robustness) are measured on training set, wheres 
(e)-(h): The metrics are measured on test set.
}
\label{fig:sensitivity-SGD}
\end{figure*}

\begin{figure*}[h!]
\centering
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_logits-generalization-adam.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_sigmoid-generalization-adam.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_logits-generalization-adam.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_sigmoid-generalization-adam.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_logits-generalization-adam-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_sigmoid-generalization-adam-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_logits-generalization-adam-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_sigmoid-generalization-adam-on-test.png}}
\caption{The correlation between input sensitivity, robustness and generalization on MNIST, $|S|=500, |E|=1000$. The optimizer is Adam. Architecture: FCN.
Here "logits" means the we use the output before the final activation (softmax or sigmoid in binary dataset).
(a)-(d): The metrics (sensitivity and robustness) are measured on training set, wheres 
(e)-(h): The metrics are measured on test set.
}
\label{fig:sensitivity-Adam}
\end{figure*}

\begin{figure*}[h!]
\centering
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_logits-generalization-entropySGD.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_sigmoid-generalization-entropySGD.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_logits-generalization-entropySGD.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_sigmoid-generalization-entropySGD.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_logits-generalization-entropySGD-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/sensitivity_sigmoid-generalization-entropySGD-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_logits-generalization-entropySGD-on-test.png}}
\subfigure[]{\includegraphics[width=0.24\linewidth]{pics/robustness_sigmoid-generalization-entropySGD-on-test.png}}
\caption{The correlation between input sensitivity, robustness and generalization on MNIST, $|S|=500, |E|=1000$. The optimizer is Entropy-SGD. Architecture: FCN.
Here "logits" means the we use the output before the final activation (softmax or sigmoid in binary dataset).
(a)-(d): The metrics (sensitivity and robustness) are measured on training set, wheres 
(e)-(h): The metrics are measured on test set.
}
\label{fig:sensitivity-Entropy-SGD}
\end{figure*}
\fi

==> experiments.tex <==
%\section{Experimental results}
%\label{sec:experiments}
In order to investigate the relationship between local flatness, volume and generalization, 
we trained DNNs on a variety of datasets including the Boolean system (see Section \ref{sec:Boolean system}),
binarized MNIST \citep{lecun1998gradient} and CIFAR-10 \citep{krizhevsky2009learning}.
The work-flow is: 
we randomly initialize the DNN, train it
until it reaches zero error on the training set, then
calculate the flatness of minima (using several different metrics described in section \ref{sec:metric of flatness}), volume of the function and generalization performance and tested their correlations 
(In Boolean system we use all samples as training set so generalization is not involved).
For volume calculation, there are two cases:
(a) on Boolean system, we randomly sample the parameters and count the empirical frequency of each functions to get their volume;  
(b) on binarized MNIST and CIFAR-10, we used neural network Gaussian Process (GP) with Expectation Propagation (EP) approximation. The detailed methodology of GP is given in section \ref{sec:GP}.
Considering the large expense of computing flatness and volume, we adopted a two hidden-layer fully connected network (FCN) with 40 ReLU units each. 
In all binary classification tasks cross entropy (CE) loss was used.

\subsection{Gaussian Process Approximation of the Volume}
\label{sec:GP}

First we introduce the methodology of using neural network Gaussian Process \citep{lee2017deep, matthews2018gaussian, tanexpectation, rasmussen2003gaussian} 
to calculate the volume of a function $V_f$.
Neural network GPs have been shown to accurately approximate the prior over
functions $P(f)$ of finite-width Bayesian DNNs \citep{valle2018deep, matthews2018gaussian}.

In the GP limit of DNNs, we can place a GP prior on the pre-activations $z$ of the last
layer of the neural network (before a final non-linearity, e.g. softmax, is
applied),
meaning that for any finite
inputs set $X=\left\{x_{1}, \ldots, x_{m}\right\}$, the random output vector (pre-activations)
$\boldsymbol{z}=\left[z\left(x_{1}\right), \ldots, z\left(x_{m}\right)\right]^{T}$ has a Gaussian distribution. 
Without loss of generality, we can assume such a process has a zero mean.
The prior probability of the outputs $\boldsymbol{z}$ can be calculated as:
\begin{equation}
P(\boldsymbol{z})=\frac{1}{(2 \pi)^{\frac{d}{2}} \Sigma^{\frac{1}{2}}} \exp \left(-\frac{1}{2} \boldsymbol{z}^{T} \Sigma^{-1} \boldsymbol{z}\right)
\end{equation}
$\Sigma$ is the covariance matrix (often called as kernel), whose entries are defined as 
$\Sigma(x_i,x_j) \equiv \mathbb{E}[z(x_i),z(x_j)]$. $d$ is the dimension of the pre-activations.
\citet{neal1994priors} gave the basic form of kernel $\Sigma$ in single hidden layer case,
where $\Sigma$ depends on the variance of weights and biases ($\sigma_w$ and $\sigma_b$). 
In DNNs with multiple hidden layers, the kernel for layer $l$ can be calculated recursively by induction, assuming the layer $l-1$ is a GP \citep{lee2017deep}. 
Particularly, the kernel for fully connected ReLU-activated networks has a well known analytical form
known as the \emph{arc-cosine kernel}
\citep{cho2009kernel}, which is the one we used in our work.

After calculating $P(\boldsymbol{z})$ with the arc-cosine kernel, the prior over (coarse-grained) functions $P(f)$ can be calculated through likelihood $P(f|\boldsymbol{z})$. We used Expectation Propagation (EP) algorithm for the approximation of $P(f|\boldsymbol{z})$ \citep{rasmussen2003gaussian}.
We represent the function $f$ by the input-output pairs on the concatenation of training set and test set $(|S|+|E|)$.
%as described in section \ref{sec:representation of functions}.
%Note here we use bold symbol $\boldsymbol{f}$ to emphasize it is a vector. By definition \ref{def:representation of functions}, $\boldsymbol{f}$ is just $f$ that we represent a function.
\begin{figure}[h!]
\centering
  \includegraphics[width=\linewidth]{pics/Sharpness-volume_bool-log10.png}
  %\label{fig:sub2}
\caption{The correlation between flatness/sharpness and volume in Boolean system.
The neural network has 7 Boolean inputs, two hidden layers of 40 ReLU units each, and a
single Boolean output.
We first built the 128-string function dataset by random sampling the parameters under initialization 
$\sigma_w = 1.0, \sigma_b = 0.1$ for $10^8$ times.
Then we 
train the network to reach zero training error using SGD and
calculated the \textbf{logarithm} of 
 Keskar-sharpness
as well as the corresponding
probability of the top-1000 most frequently-appearing functions. The volume $V_f$ here is exactly what we defined in definition \ref{def:volume}, without coarse-graining. 
Note that the reason why we have two bands is because of the flatness discontinuity of Boolean functions, i.e. functions which have $n$ and $n+1$ outliers will show a discontinuity of flatness. We say there is 1 outlier if there is a single "1" with 127 "0"s or a single "0" with 127 "1"s. 
}
\label{fig:bool}
\end{figure}
\subsection{The correlation between flatness and volume}
\label{flatness-volume correlation}

%Intuitively, it is not hard to imagine that a flatter loss landscape will enclose a bigger volume in the parameter space. Because the change of the loss is relatively slow,
%one needs to perturb further in order to jump out of the neutral space.  
In this subsection, we provide numerical evidence to show that flatness and volume can be related.
When they do correlate, the flatness serves as local approximation to volume. This possible correlation is what behind the common (but rough) belief that flat minima generalize better.
%when the optimizer does not have preference for flatter minima (e.g. SGD). 
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/MNIST-sharpness-generalization-log10.png}
  \caption{}
\end{subfigure} 
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/MNIST-volume-generalization-log10.png}
  \caption{}
\end{subfigure} 
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/MNIST-sharpness-volume-log10.png}
  \caption{}
\end{subfigure}
\caption[Caption for LOF]{The correlation between Keskar-sharpness, volume $V_f$ and generalization accuracy on binarized-MNIST.
The training set size is 500; the attack-samples size range from (0 - 500) in order to get different generalization performance. Test set size is 1000. A 784-40-40-1 FCN\footnotemark~with He-normal initialization and SGD optimizer was used. 
We trained neural networks with different size of attack set till reaching zero training error and calculated corresponding metrics.
%\textbf{Note: all sharpness and volume measures are logarithm.}
{\em (a)} Sharpness v.s. generalization performance. 
{\em (b)} Volume v.s. generalization performance. Here the volume is calculated using the GP-EP approximated volume on the concatenation of genuine training set and test set.
{\em (c)} The correlation between local sharpness and volume.
}
% \ard{if you instead take the sharpness after say after 100 or other number of  epochs of overtraining does it correlate better or worse with volume and generalization?}

\label{fig:MNIST}
\end{figure*}
\subsubsection{Boolean system}
\label{sec:Boolean system}
We first build a prototypical neural network consisting of 7 Boolean inputs, 2 hidden layers with 40 ReLU
neurons each and a single Boolean output.
This architecture has been found to be sufficiently
expressive to represent almost all possible output functions \citep{valle2018deep}. We randomly sample the network’s weights and biases for $10^8$ times and measure the output (denoted as 0 or 1). 
The initial standard deviation is $1$ for weights and $0.1$ for biases ($\sigma_w =1, \sigma_b = 0.1$).
By this process, the function that the DNN is expressing
can be represented as a 128 bit string, with each bit corresponding to the Boolean output for
one of the $2^7$ possible inputs. 
%By simply counting the empirical frequency of each output string, 
By using equation \ref{equation:volume},
we can
estimate the volume each function.

Next, we train our network with SGD using the same initialization to produce the top-1000 most commonly appearing output functions (with zero training error) and then evaluate two kinds of flatness measure: {\em (a)} the spectral norm of Hessian $\lambda_H^1$
and {\em (b)} logarithm of Keskar-sharpness in equation \ref{equ:keskar-sharpness} with an $\epsilon$ of $10^{-4}$. 
For the maximization process in calculating Keskar-Sharpness, we run SGD for 100 epochs and make sure the max value ceases to improve. 
As
Figure \ref{fig:bool} demonstrates, both flatness metrics are strongly correlated with the volume
$V_f$. It appears that flatness, the conventional explanation of DNN generalization properties, is
serving as a proxy for the more fundamental and theoretically corroborated quantity of volume.



\subsubsection{MNIST and CIFAR-10}
\label{sec:MNIST and CIFAR-10}
Now we want to see how flatness and volume correlate with generalization performance on real-life dataset. 
We use a feed-forward network with 784 input nodes (corresponding to each
of the image pixels) and two further hidden layers with 40 ReLU nodes each.
For simplicity, We use binarized-MNIST by simply marking class (0-4) as ``0" and (5-9) as ``1". As for CIFAR-10 we choose two categories out of ten: cars and cats. We restrict our training set to be small (500/5000 for MNIST/CIFAR-10). Experiments with bigger training set are 
done but not shown in this report.
% shown in Appendix. \ref{appendix:larger training set}.

In order to compare solutions with very diverse generalization
performances (i.e. from solutions that as good as above $90\%$ accuracy to solutions as
poor as a random guess), we borrowed the attack-set trick implemented by \citet{wu2017towards}: 
The attack-set consists of attack-samples which are normal pictures but labelled wrongly deliberately.  
%corrupting the training set with additional ``attack-set" which contains normal pictures but with flipped labels, and then train to $100\%$ accuracy. 
The system with corrupted training set is then trained to zero error.
It is straightforward that the more attack-samples get mixed into genuine training set, the worse the DNN generalizes. Thus
we can tune the generalization performance by adding different size of attack-set.

After training the corrupted training set to $100\%$ accuracy, we calculate the flatness and volume while testing the generalization performance on the test sets. Given the similarity between Hessian-based metrics and Keskar-sharpness,
%(See Figure \ref{fig:self-similarity-1} and \ref{fig:self-similarity-2})
we only present the latter one because of the $O(n^2)$ heavy computing cost for the Hessian. 
The same setting of $\epsilon$ and maximizing epochs as in section \ref{sec:Boolean system} are used. 
% More Hessian-based results can be seen in Appendix \ref{appendix:hessian based}. 
The volume is calculated with GP-EP approximation using the \texttt{GPy} package \citep{gpy2014}, while the inputs and outputs (labels) being 
$(\mathtt{concat}(X_{genuine}, X_{test}), \mathtt{concat}(\mathbf{y}_{genuine}, f(X_{test})))$.
Here $\mathtt{concat}$ means concatenation. 
As demonstrated in Figure \ref{fig:MNIST} (MNIST) and \ref{fig:cifar10} (CIFAR-10), volume is a loyal predictor of the generalization performance; sharpness keeps its correlation with volume (hence generalization). Again, SGD optimizer was used here. 


\footnotetext{Here the four digits are number of input nodes, first hidden layer nodes, second hidden layer nodes, output nodes, respectively.}
\begin{figure*}[p]
\centering
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/cifar10-sharpness-generalization-log10.png}
  \caption{}
  \label{fig:mnist-sharpness-generalization}
\end{subfigure} 
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/cifar10-volume-generalization-log10.png}
  \caption{}
\end{subfigure} 
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{pics/cifar10-sharpness-volume-log10.png}
  \caption{}
\end{subfigure}
\caption[Caption for LOF]{
The correlation between Kerkar-sharpness, volume $V_f$ and generalization accuracy on two categories of CIFAR-10: cat and car.
There are 10000 pictures in these two categories, in which 5000 pictures have been chosen as training samples; we flipped the labels of the other 5000 pictures and used them at attack-set. Test set size is 2000. A 3072-40-40-1 FCN\footnotemark~with He-normal initialization and SGD optimizer was used. 
%We kept training until zero training error was reached. 
%\textbf{Note: all sharpness and volume measures are logarithm.}
{\em (a)} Sharpness v.s. generalization performance. 
{\em (b)} GP-EP approximated volume v.s. generalization performance. 
{\em (c)} The correlation between local sharpness and volume.
}
\label{fig:cifar10}
\end{figure*}
\footnotetext{3072 is the number of input nodes.}
\subsection{Time evolving behavior of sharpness and volume}

In experiments above, flatness and volume metrics are calculate one-off upon reaching $100\%$ training accuracy. However, in order to show that volume is a robust global metric and hence superior than flatness, we need to know how they evolve with epochs. To this end, we run the same FCN as in Figure \ref{fig:MNIST} on binarized-MNIST again, but this time we calculate sharpness and volume at each epoch.

As described in section \ref{sec:re-scaling}, the function found by the DNN should be unchanged under reparameterization such as $\alpha$-scaling. To test what this means for volume and flatness measures, we first wait for 500 epochs after achieving $100\%$ training accuracy, and then we manipulate the weights and biases of the two hidden layers to trigger the $\alpha$-scaling. 
As shown in Figure \ref{fig:evolve}, sharpness drops and plateaus once reaching $100\%$ training accuracy, shoots up upon $\alpha$-scaling, then relaxes back down again. By contrast, volume remains stable throughout, and particularly does not change when the $\alpha$-scaling happens because the optimizer does not leave the neutral 
space in Figure \ref{fig:5.1};
Or, as can be seen in Figure \ref{fig:5.9}, if the perturbation is large enough, then the volume temporarily changes because SGD acts on gradients, and right after $\alpha$-scaling these can be large enough to "knock" the optimiser to a different function. However, in just a few steps, the system converges back to the original function and volume.
%or make a foray into a neighbouring subspace due the random nature of SGD
%and the very steep character (big gradients) of the loss after re-scaling (Figure \ref{fig:5.9}). 
It is clear that
$\alpha$-scaling can change the flatness nearly arbitrarily, and it keeps changed onward.
However, even if the re-scaling parameter is big enough to drive the optimizer out of current neutral space, it will still come back very quickly.

Here we need to clarify that after reaching 100\% accuracy on training set, the training loss, on which SGD is trained on, can still drop.
As an example, consider an output unit with value $0.6$ and $0.8$ while the true label being $1$: they both correctly predict the label (same accuracy), but the $0.8$ case has lower cross entropy loss.  
Moreover, the sharpness is also dropping after reaching 100\% training accuracy, meaning the optimizer generally keeps finding flatter region even in the same basin of function.  

\begin{figure}[htbp]
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{pics/sharpness-volume-evolve-volume-doesnot-change-log10.png}
  \caption{}
  \label{fig:5.1}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{pics/sharpness-volume-evolving-log10.png}
    \caption{}
    \label{fig:5.9}
\end{subfigure}
\caption{The sharpness and volume evolving with epochs in the post-training regime. Green dashed line means zero-training error is reached and post-training starts; 
\textbf{red dashed line means $\alpha$-scaling takes place
($\sim$ 620th epoch)
.} The architecture is 2 hidden-layer FCN, trained on binarized-MNIST with train/test set size being 500/100. He-normal initialization was used. 
GP-EP approximated volume $V_f$ and Keskar-sharpness are calculated as the end of each epoch. 
{\em (a)} When the re-scaling parameter $\alpha$ is not ``big enough" ($\alpha = 5.0$), an instant change of sharpness can be seen when re-scaling takes place, but the optimizer does not jump out of the neutral space, thus there is no change in volume on the epoch where re-scaling happens.
{\em (b)} When $\alpha$ is ``big enough" ($\alpha = 5.9$), the re-scaling manipulation not only changes the sharpness immediately, but also introduces big gradients for the optimizer to jump out of the neutral space. It then goes back to the same level of volume very quickly. 
}
\label{fig:evolve}
\end{figure}

\subsection{Comparison between optimizers}
\label{sec:comparison between optimizers}

A lot of algorithms are designed to bias the optimizer into flatter regions explicitly (encoded in the loss function) \citep{hochreiter1997flat,chaudhari2019entropy} or implicitly
(encoded in the learning dynamic)
\citep{kingma2014adam}. However, recent works have shown that these imposed flatness preference not necessarily bring in better generalization \citep{keskar2017improving,wilson2017marginal}. 
Intuitively, we assume that SGD samples parameters close to uniformly within the neutral space, i.e. it has no preference for flatter weight configurations when expressing the same function. Under this assumption, from Figure \ref{fig:MNIST} we can see that on average, local sharpness correlates well with generalization accuracy.
A question we then want to ask is \textbf{``Does that mean flatness-generalization correlation breaks down when using these biased SGD-variants?"} The answer is yes.

In order to see this, we choose two SGD-variants: Entropy-SGD 
(with explicit bias towards flatter minima) \citep{chaudhari2019entropy}
and Adam. 
We then use these optimizers to train our FCN into $100\%$ training accuracy. We then calculate the sharpness and volume upon reaching target accuracy and observe their correlation with generalization. Figure \ref{fig:comprasion-a},\ref{fig:comprasion-b},
\ref{fig:comprasion-d}
,\ref{fig:comprasion-e} are under the exact same conditions (on MNIST with same architectures, hyperparameters etc.) as Figure \ref{fig:MNIST} except for the optimizer, so are Figure \ref{fig:comprasion-c}, \ref{fig:comprasion-f} and Figure \ref{fig:cifar10} on CIFAR-10. As seen in Figure \ref{fig:optimizers}, when the optimizer has inherent bias for the characteristic of minima it finds, the correlation between flatness and generalization severely deteriorates.
As an example, 
compared with vanilla SGD in Figure \ref{fig:mnist-sharpness-generalization}, 
the Entropy-SGD and Adam optimizer in Figure \ref{fig:comprasion-a},\ref{fig:comprasion-b} will always try to find flatter minima, even for those poorly generalized functions. The volume, however, always correlates nicely with generalization no matter if the optimizer is biased or not.
These results have further shown that as a local quantity, flatness does not necessarily correlate with generalization ability, but volume always does.
\begin{figure}[htbp]
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/sharpness-generalization-entropy-sgd-log10.png}
      \caption{}
      \label{fig:comprasion-a}
    \end{subfigure}%
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/sharpness-generalization-adam-log10.png}
      \caption{}
      \label{fig:comprasion-b}
    \end{subfigure}%
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/sharpness-generalization-cifar10-adam-log10.png}
      \caption{}
      \label{fig:comprasion-c}
    \end{subfigure}%
    \\
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/volume-generalization-entropy-sgd-log10.png}
      \caption{}
      \label{fig:comprasion-d}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/volume-generalization-adam-log10.png}
      \caption{}
      \label{fig:comprasion-e}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{pics/volume-generalization-cifar10-adam-log10.png}
      \caption{}
      \label{fig:comprasion-f}
    \end{subfigure}
    \caption{
    SGD-variants break down the flatness-generalization correlation.
    When using these biased-towards-flatter-minima optimizers, the correlation between sharpness and generalization performance  can no longer exist, but the volume $V_f$ keep correlating with generalization. \\
    {\em (a)} and {\em (d)}: Shaprness v.s. generalization and volume v.s. generalization with Entropy-SGD on binarized-MNIST. The setting is the same with Fig.~\ref{fig:MNIST} except for the optimizer. \\
    {\em (b)} and {\em (e)}: Adam optimizer on binarized-MNIST.  The setting is the same with Fig.~\ref{fig:MNIST} except for the optimizer. \\
    {\em (c)} and {\em (f)}: Adam optimizer on CIFAR-10. The setting is the same with Fig.~\ref{fig:cifar10} except for the optimizer.  
    %\ard{question: try to make the x and y axes the same for the MNIST. }  \\
    % \ard{If you overtrain, is the sharpness-generalisatino correlation better?} 
    }
    \label{fig:optimizers} 
\end{figure}




==> paper_overview.tex <==
% \section{Overview for the concept "flatness"}


The concept "flatness" of loss function of neural networks can be traced 
back to \citet{hinton1993keeping} and \citet{hochreiter1997flat}.
%The intuition is very straightforward, as described in figure 
%\ref{fig:flat_minima}.
Although they did not provide a formal mathematical
definition of flatness, \citet{hochreiter1997flat} described a flat minima as "a large connected region in parameter space where the loss remains approximately constant", which requires low 
precision to specify than a sharp minima.
They linked to 
the minimum
description length (MDL) principle \citep{rissanen1978modeling},
which says the best performing model is the one with shortest description length,
to argue that flatter minima should generalise better than sharp minima. 
To take this into account, they suggested 
 adding a extra regularization term to the original loss function in order to drive the optimizer into finding those minima that need less information to specify (i.e. flatter minima).
The new loss function can be formalized as: 
\begin{equation}
L^\prime \left(\mathbf{w}\right)=L\left( \mathbf{w} \right)+ \lambda \sum_{x_{i} \in X} B\left(\mathbf{w}, x_{i}\right).
%\lambda B\left(w, X_{0}\right)
\end{equation}
where the regularization terms $B\left(\mathbf{w}, x_{i}\right)$ can be naively understood as the "bits of information" needed to encode the minima, $\lambda$ is the hyperparameter which controls the trade-off between training error and regularization. They empirically showed that working on this modified loss function would outperformed vanilla loss.    
\iffalse
A similar work done by \citet{chaudhari2019entropy} also introduced an extra regularization to bias the optimizer into wider valleys. Instead of minimizing the original loss, they proposed to maximize the "local entropy":
\begin{equation}
L^\prime(\mathbf{w})=\log \int_{\mathbf{w}^{\prime} \in \mathbb{R}^{n}} \exp \left(-L\left(\mathbf{w}^{\prime}\right)-\frac{\lambda}{2}\left\|\mathbf{w}-\mathbf{w}^{\prime}
\right\|_{2}^{2}\right) d \mathbf{w}^{\prime}
\label{eq:local-entropy}
\end{equation}
in which $\mathbf{w^\prime}$ is also parameter vector but needs to be integrated out. 
The "local entropy" smooth the loss landscape and penalize those minima which have low loss but their neighbors have high loss, i.e. sharp minima.
\fi

%Above regularization methods both can drive optimizer into flatter minima, but neither of them defined a calculable metric of flatness.
The first detailed practical measurements of flatness was given in an influential paper \citep{keskar2016large}, in the context of investigating the generalization gap between large-batch and small-batch training. 
The batch size refers to the number of training examples utilized in a single iteration of stochastic gradient descent (SGD), the most used optimisation method for DNNs.  As opposed to simple gradient descent (GD), in SGD a stochastically chosen subset of training data (the batch) is used to set the gradients at each time-step.
The generalization gap here refers to the phenomenon that large-batch training 
%with SGD (or its variants like Adam or Adagrad) 
tends to have slightly worse generalization ability (from $\sim 0.2 \% $ to $\sim 5 \%$) compared to small-batch training, even if they can achieve similar performance on training set.

\citet{keskar2016large} claim that the generalization gap arises because large-batch methods tend to converge
to sharp minima of the training loss function, while small-batch methods are more prone to flat minima.
%Figure \ref{fig:keskar-flat-minima} gives a very intuitive conceptual diagram of understanding why flat minima tend to generalize better:
%flat minima are more robust when there is a discrepancy between training loss and test loss (which is almost always the case), which prevent the model from being deteriorated too much; sharp minima are corresponding to large sensitivity, which negatively impacts the ability of the trained model to generalize on new data.
%\begin{figure}
%    \centering
%    \includegraphics[width=1\linewidth]{pics/Keskar-flat-minima.png}
%    \caption{A conceptual sketch of flat and sharp minima. The x-axis indicates the weights configuration and the y-axis is the value of loss function. When there is a discrepancy between training loss function and testing loss function (this discrepancy usually originates from the data distribution difference), the flat minima trained on training function perform similar on testing function, while the sharp minima perform fairly poor on testing function. \ard{Figure from~\citep{keskar2016large}}}
    \label{fig:keskar-flat-minima}
%\end{figure}
%Keskar et al.  \ard{in LATEX use $\\ $ after $.$ that is not end of a sentence to get rid of extra space}
Perhaps the most natural way to measure the flatness of minima is to consider the eigenvalue distribution of the $H_{ij} = \partial^2L(\mathbf{w}) / \partial w_i \partial w_j$ once the learning process has converged (typically to a zero training error solution). Sharp minima are characterized by a significant number of large positive eigenvalues in the Hessian, while flat minima have numerous small eigenvalues (Note that some care must be used in this interpretation because it is widely thought that DNNs converge to stationary points that are not true minima). However, Hessians are typically very expensive to calculate. Thus \citet{keskar2016large} used a computationally more tractable measure they call "sharpness". 
%They also mentioned that one characterization of flatness of minima is the eigenvalue distribution of loss Hessian: sharp minima are characterized by a significant number of large positive eigenvalues in the Hessian, while flat minima have numerous
%small eigenvalues. 
%The Hessian is the second order derivative matrix of loss w.r.t. parameters:
%$H = {\partial ^2 L(\mathbf{w})} /{\partial \mathbf{w}^2}$ .
%However, given the prohibitive cost of Hessian calculation, they did not adopt Hessian as the measure of sharpness, but defined a computationally feasible sensitivity measure of sharpness. 
It is based on exploring a small neighborhood
of a minimum and computing the largest value that the loss function $L(\mathbf{w})$ can attain in that neighborhood.
%In order to avoid being mislead by the case when a large
%value of $L(\mathbf{w})$ only exists in a tiny subspace of $\mathbb{R}^{n}$, the maximization process is performed both in the entire
%space $\mathbb{R}^{n}$ as well as in random manifolds. 
%For that purpose, a random matrix $A$ is introduced, whose
%columns are randomly generated and has dimension $n \times p$, $n$ is the dimension of parameter space and $p$ determines the dimension of the manifold. Keskar et al. set $p = 100$ in their experiments.
%\sofun{define my own version without A}
Let $\mathcal{C}_{\epsilon}$ denote the box around the minimum of interest where the maximization of $L(\mathbf{w})$ is performed; $\epsilon$ is a hyperparameter that controls the size of the box. 
The box boundary $\mathcal{C}_{\epsilon}$ is defined as:
\begin{equation}
\mathcal{C}_{\epsilon}=\left\{\Delta \mathbf{w} \in \mathbb{R}^{n}:-\epsilon\left(\left| w_{i}\right|+1\right) \leq \Delta w_{i} \leq \epsilon\left(\left| w_{i}\right|+1\right) \quad \forall i \in\{1,2, \cdots, n\}\right\}
\end{equation}
With the box boundary, the measure of sharpness can be defined:
\begin{definition}{Keskar-sharpness:}
Given $\mathbf{w} \in \mathbb{R}^{n}$ and $\epsilon>0$, define the $\mathcal{C}_{\epsilon}$-sharpness of $L(\mathbf{w})$ at parameter $\mathbf{w}$ as: 
\begin{equation}
\mathrm{sharpness}:=\frac{\left(\max _{\Delta \mathbf{w} \in \mathcal{C}_{\epsilon}} L(\mathbf{w}+\Delta \mathbf{w} )\right)-L(\mathbf{w})}{1+L(\mathbf{w})} \times 100
\label{equ:keskar-sharpness}
\end{equation}
\end{definition} 
\par \noindent
This measure of sharpness is closely related to the spectral norm of $\nabla^{2} L(\mathbf{w})$: assuming $\epsilon$ to be small enough, consider the second order Taylor expansion of $L(\mathbf{w})$ around a critical point minima $\mathbf{w}$
\begin{equation}
L\left(\mathbf{w}^{\prime}\right)= L(\mathbf{w})+\frac{1}{2}\left(\mathbf{w}^{\prime}-\mathbf{w}\right)^{T}\left(\nabla^{2} L(\mathbf{w})\right)\left(\mathbf{w}^{\prime}-\mathbf{w}\right) \\
+o\left(\left\|\mathbf{w}^{\prime}-\mathbf{w}\right\|_{2}^{2}\right)
\end{equation}
where $\mathbf{w}^\prime$ is the updated parameter found by the maximizing process. The sharpness metric in equation \ref{equ:keskar-sharpness} at the critical point can be written using the spectral norm:
\begin{equation}
\mathrm{sharpness} = \frac{\left\|\left|\left(\nabla^{2} L(\mathbf{w})\right)\right|\right\|_{2} \epsilon^{2}}{2(1+L(\mathbf{w}))} \times 100
\end{equation}
%Using this metric of flatness, the authors provided numerical evidence that convergence to sharp
%minima gives rise to the poor generalization of large-batch methods for deep learning. 
% \textbf{Wu et al.}(2017) \\ \\
\citet{keskar2016large} used the L-BFGS-B algorithm~\citep{byrd1995limited} to perform the 
maximization of $L(\mathbf{w})$ in $\mathcal{C}_{\epsilon}$. However, as a quasi-Newton method, L-BFGS-B is not scalable when there are tens of millions of parameters in modern DNNs. To make Keskar-sharpness applicable for large DNNs, we will use SGD for the maximization instead.

Some researchers adopted eigenvalue-based measure for flatness. 
\citet{wu2017towards} argue that local flatness described by Hessian eigenvalues is a proxy for the volume of basin of attractor; the latter one they claimed to be decisive of whether the attractor leads to good generalization. 
For the local flatness measure, they used either the log-product of top-$k$ Hessian eigenvalues
if the size of DNN is manageable, 
or statistical estimate of the Frobenius
norm of Hessian if direct calculation of Hessian is out of reach. Similarly, \citet{zhang2018energy} borrowed the conception of energy–entropy competition from physics, treating mean training loss as "internal energy" and flatness as "entropy";
they then approximated the entropy as the log-product of Hessian eigenvalues. 
\citet{yao2018hessian} also investigated the generalization gap induced by large batch training 
from a robust training perspective, 
and found
that 
the local flatness, quantified by the spectral norm of Hessian, can be predictive of how likely the model would be affect by adversarial samples attack. 
% \sofun{PAC-Bayesian flatness measure Jiang et al.}
Most recently, \citet{maddox2020rethinking} revisited the effective dimensionality of Hessian and found they can also relate this measure to local flatness. 

\subsection{Re-scaling Problem}
\label{sec:re-scaling}
All the above measures of flatness seem quite promising: correlation between "flat" minima and better generalization performance were found in different notions of flatness. 
However, \citet{dinh2017sharp} argued that all these notions of flatness are problematic for deep neural networks and can not be directly applied to explain generalization. 
%They provided evidence that the concept of flat minima is not well defined,
%which requires rethinking
%what flatness actually means.
The main logic behind the argument is that over-parametrized DNNs exhibit a large number of different parameter configurations which result in exactly the same function; but these parameter configurations may have different values of flatness. 
Take a single-hidden-layer ReLU activated network as an example:
$$\hat{Y}=\phi_{\mathrm{ReLU}}\left(X \cdot \mathbf{w_{1}}\right) \cdot \mathbf{w_{2}}$$
where $\mathbf{w_1}$ are weights between input layer and hidden layer and $\mathbf{w_2}$ are weights between hidden layer and output layer 
(note for convenience we can exclude the bias terms).
$\phi_{\mathrm{ReLU}}$ is the rectified linear function: 
$\phi_{\mathrm{ReLU}}(x) = \max (0,x)$.
    "Equivalent" parameter configurations can be easily achieved by "$\alpha$-scaling" transformation: 
$$T_{\alpha}:\left(\mathbf{w}_{1}, \mathbf{w}_{2}\right) \mapsto\left(\alpha \mathbf{w}_{1}, \alpha^{-1} \mathbf{w}_{2}\right)$$
%T_{\alpha}$ denotes the family of parameter transformation.
Note that a "$\alpha$-scaling" transformation will not change the generalization performance of the neural network, because the DNN still represents the very same function after transformation. Also, this idea of parameter transformation without changing the representing function can be trivially extended to any architecture having a single ReLU activated network as a submodule.
It can be further proved that after "$\alpha$-scaling" transformation, both Keskar sharpness and the Hessian-based measure of flatness 
can change arbitrarily, while the generalization performance stays the same.

% \textbf{Scale invariant Flatness measures} \\ \\
In light of the existence of "$\alpha$-scaling" problem, several recently works have been focusing on finding a "scale invariant" flatness metric. 
\citet{petzka2019reparameterization}, \citet{rangamani2019scale} and \citet{tsuzuku2019normalized}
have all proposed a new "scale invariant" Hessian-based flatness measure separately,
but the idea behind them is similar. The trick is simply multiplying layer-wise Hessian eigenvalues by a factor of $\|\mathbf{w_i}\|^{2}$, then the new metric is immune to layer-wise reparameterization. 
%The intuitive way of understanding this phenomenon is:
%"$\alpha$-scaling" will rescale the norm of layer-wise weights;
%however, we can come up with a new metric which has already contained the information of norm, then
%after the rescaling process imparted by "$\alpha$-scaling", the total scaling effect will cancel off, which makes this new metric scale-invariant.
The new scale invariant metric looks promising experimentally, however, this metric is only scale-invariant when it is layer-wise.
Also, "$\alpha$-scaling" is not the only way of reparameterization, but just a particular case where layer-wise weights are changing collectively. As long as the optimizer goes into the neutral space (which is defined in section \ref{sec:neutral space}), there is much more possibilities for "irregular" reparameterization. Therefore, it seems that these "scale invariant" metrics have not reached the real core of the reparameterization problem.


==> volume.tex <==
\subsubsection{The Parameter-function Map}
With the representation of functions, we then introduce the definition of the parameter-function map \citep{valle2018deep,mingard2020sgd}:
\theoremstyle{definition}
\begin{definition}[Parameter-function map]
Consider a parameterised supervised model, and
let the input space be $\mathcal{X}$ and the output space be 
$\mathcal{Y}$. The space of functions the model can
express is a set 
$\mathcal{F} \subseteq \mathcal{Y}^{|\mathcal{X}|}$.
If the model takes parameters within a set
$W \subseteq \mathbb{R}^{n}$,
then the parameter-function map $\mathcal{M}$ is defined as 
$$\begin{aligned}
\mathcal{M}: W & \rightarrow \mathcal{F} \\
\mathbf{w} & \mapsto f(\mathbf{w})
\end{aligned}$$
\label{def:para-func map}
\end{definition}
The parameter-function map serves as the bridge between parameter-space searching algorithm (e.g. SGD) and its  behavior in function space. The latter 
determines the generalization ability of model.
As mentioned before, for dataset where the input space $\mathcal{X}$ is too large for our calculations to be feasible, we often restrict the inputs to a subset of original input space. 

% I dont think we'll use this notation below really, so unecessary.
% If we want to make explicit in notation which subset we are using for a parameter-function map, we will use the notation $f_\theta(X)$ to represent the restricted function that the network with parameters $\theta$ expresses, restricted to $X$.

%Mathematically, the volume of the set of parameters mapping to a specific function is measured by the marginal likelihood $p(\mathbf{y}|X)$, where $X$ and $\mathbf{y}$ are the inputs and outputs of the DNN corresponding to the specific function, while $\theta \in \Theta_\mathcal{N}$
%  $S = (X, \mathbf{y}) \in \mathcal{X}\times\mathcal{Y}$
% given dataset (i.e. input-output pairs), 

\subsubsection{The Neutral space}
\label{sec:neutral space}
Before deriving the concept of "volume of functions", we introduce the definition of \emph{neutral space}, which is defined as the
set of parameters mapping to a specific function. 
\begin{definition}[Neutral space]
For a model defined in Definition \ref{def:para-func map},
%input $X\in \mathcal{X}$ and label $\mathbf{y} \in \mathcal{Y}$, 
and a given function $f$, the neutral space $\mathcal{N}_f \subseteq W$ is defined as
$$
\mathcal{N}_f := \{ \mathbf{w} \in W : 
\mathcal{M}(\mathbf{w}) = f \}
$$
\label{def:neutral space}
\end{definition}
% Note that the neutral space is dataset (function)-specified and can have infinite elements.
The size of neutral space can be informally defined as the volume of the corresponding function. 
Note that the neutral space may be unbounded. In those cases, the "size" of neutral space might be counterintuitive at the first glance. However a probabilistic measure of the set may still be defined. We will use this probabilistic measure as the starting point for our Bayesian formalization.

\subsubsection{The Bayesian Prior, Posterior and Volume}
\label{sec:volume and Bayesian posterior}
In this section we give the definition of volume as well as its relationship with the Bayesian picture.
We define the ``volume of a function $f$'' as a probabilistic measure of its neutral space:
\begin{definition}[Volume of a function]
Given the prior distribution $P(\mathbf{w})$ over the parameters, the \emph{volume of function $f$}, $V_f$, can be defined as:
\begin{equation}
V_f:=P(f)=P(N_f)=\int \mathbbm{1}[\mathcal{M}(\mathbf{w})=f] P(\mathbf{w}) d \mathbf{w}
\label{equation:volume}
\end{equation}
\label{def:volume}
\end{definition}

where $\mathbbm{1}$ is an indicator function:
$\mathbbm{1}[arg] = 1$ if its argument is true or $0$ otherwise.
$V_f$ can be interpreted as the probability of the DNN expressing function $f$ upon initialization (i.e. before an optimization process). We will also refer to this quantity as $P(f)$, 
because it can be interpreted as a Bayesian prior over functions, as done in \cite{valle2018deep,mingard2020sgd}.
%of coarse-graining
%we mentioned at the beginning of section \ref{volume}.
%With this prior, 
If we condition functions on obtaining zero prediction error on  training set 
$S=(X,Y)$, we have the Bayesian posterior 
\begin{equation}
P(f \mid S):=\frac{P(S \mid f) P(f)}{P(S)}
\label{equ:posterior}
\end{equation}
In the context of supervised learning with training dataset $S=\left\{\left(x_{i}, y_{i}\right)\right\}_{i=1}^{m}$,
the term $P(S | f)$ in Equation \ref{equ:posterior}
%(which should be $P(Y|f,X)$ technically but we use 
%$P(S | f)$ to simplify notation) 
corresponds to a 0-1 likelihood
$$
P(S \mid f)=\left\{\begin{array}{l}
1 \text { if } \forall i, \quad f\left(x_{i}\right)=y_{i} \\
0 \text { otherwise }
\end{array}\right.
$$
and the normalization term (\emph{marginal likelihood}) $P(S)$ is 
$$
 P(S) = P(Y\mid X) = 
    \sum_{f} P(S \mid f) P(f)=\sum_{f \in \mathcal{C}_S} P(f) \\
    = \int_{\mathbf{w} \in \mathcal{N}_S} P(\mathbf{w}) d\mathbf{w}
$$
with $\mathcal{C}_S$ denoting the set of all functions compatible with the dataset
$S$ and $\mathcal{N}_S$ refers to the neutral space for all $f \in \mathcal{C}_S$.
The marginal likelihood can also be interpreted as the sum of "volume" of all functions  $f \in \mathcal{C}_S$.
From equation \ref{equ:posterior}, we can derive an important relationship between the posterior 
and the volume of a function:
\begin{equation}
    P(f \mid S) \propto V_f = P(f)\quad \text{if} \quad P(S \mid f)=1
\label{equ:volume-posterior relationship}
\end{equation}
 Thus the probability that a function $f$ obtains upon training a DNN to zero training error by random sampling of parameters is proportional to the "volume" of the function. In this report we will calculate the volume of the function defined on the inputs $X$ and $X^\ast$ of the training set and test set respectively. 


\subsubsection{The Heuristic Correlation Between Volume and generalization}

While \citet{wu2017towards} suggested that the volume of basin of attraction relates to 
generalization, their assumption: local flatness is a good proxy for the volume of basin of attraction,  
is not necessarily true. 
In fact,
\citet{izmailov2018averaging} have shown that even in the same basin of attraction, there can be flatter region and sharper region.
Figure. \ref{fig:volume-sharpness-scheme-plot} schematically shows our understanding of the loss landscape, in which the local flatness may not necessarily correlated to the volume of basin of attraction noted as $V_\mathrm{S G D}\left(f\right)$\footnotemark.
%In order to be more predictive, we have to find a metric which is a global quantity (so it also will not suffer from the reparameterization problem). 
However, 
the volume of "basin size", which we noted as $V_B(f)$, might be a more stable proxy for $V_\mathrm{S G D}\left(f\right)$.
Note that $V_B(f)$ is proportional to Bayesian posterior $P(f | S)$ if the function reach zero error on training set.
From what we have shown in section \ref{sec:volume and Bayesian posterior} we know that the volume of a function $V_f$ is proportional to $V_B(f)$.

%If we \emph{only} use Gaussian Process (GP) to approximate $V_f$ (see section \ref{sec:GP}), we can except that functions with high $V_f$ will have low generalization error, because Gaussian Process in general has good generalization performance. In fact, 
Recently \citet{mingard2020sgd} have empirically confirmed the correlation
between the basin size $V_B(f)$ and the volume of basin of attraction $V_\mathrm{S G D}\left(f\right)$,
by showing  
that for a range of architectures, datasets and optimizers, the probability for an optimizer to converge on a function $f$ consistent with a training set
$S$, $P_{\mathrm{SGD}}(f | S)$, correlates well with the GP-EP approximated (see section \ref{sec:GP}) Bayesian posterior probability, $P(f | S)$. 
Note that $V_\mathrm{S G D}\left(f\right) \propto P_{\mathrm{SGD}}(f | S)$  
and $V_B(f) \propto P(f | S)$.
Moreover, they have also shown in their figure 1(b) that $P(f | S)$ is exponentially biased towards
functions with low generalisation error.
Considering the relationship in equation \ref{equ:volume-posterior relationship}, we expect there is also a logarithm relationship between $V_f$ and generalization error.
\citet{mingard2020sgd} suggested that the logarithmic form of the correlation may originate from the Poisson-Binomial-like distribution over the misclassifying probabilities of individual images $p_i$,
which are independent and non-identical.

%The question is, whether functions found with high $V_f$ by optimizers like SGD (which is what we care in application) should also have low generalization error?

%Note that $P_{\mathrm{SGD}}(f | S)$ is proportional to $V_{\mathrm{S G D}}(f)$ and $P_{\mathrm{B}}(f | S)$ is proportional to $V_{B}(f)$. 
%Also, as the Bayesian posterior, $P_{\mathrm{B}}(f | S)$ is also proportional to our volume, according to equation \ref{equ:posterior}. 
%But it is still a possible scenario where both the GP and the SGD have low error, they 
%nevertheless still find different functions. 
%Thus, the correlation between $V_f$ found by optimizers and generalization is a non-trivial %prediction. 
%In this paper, we confirm this correlation exists by using attack-set (see section \ref{sec:MNIST and CIFAR-10}) to trick the optimizer to finding a series of function with very diverse generalization.  

%Thus, the correlation between 
%$P_{\mathrm{SGD}}(f | S)$ and $P_{\mathrm{B}}(f | S)$ boils down the the correlation between volume of function $V_f$ and volume of basin of attraction $V_{\mathrm{S G D}}(f)$.
%Moreover, \citet{mingard2020sgd} have shown the strong correlation between $log(P_{\mathrm{B}}(f | S))$ and generalization by manually selecting certain number of labels in the test set to be wrong.
%This discovery  
%strongly hints that we should use volume, instead of local flatness, as the global predictor of generalization.  
\footnotetext{Here the subscript "SGD" means when initial weights are in the basin of attraction, it will then be "attracted" to the bottom of basin by optimizers like SGD or its variants.}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pics/volume_and_flatness_scheme_plot.png}
    \caption{Schematic loss landscape highlighting the relationship between volume of the basin, 
    volume of the (basin of) attraction and local flatness. 
    While flatness can vary inside the same basin
    (rugged bottom), the volume of function $f_1$ ($\propto$ $V_{B}(f_1)$ ) is shown to be closed related to the volume of basin of attraction $V_{\mathrm{S G D}}(f_1)$.
    }
    \label{fig:volume-sharpness-scheme-plot}
\end{figure}


% \begin{definition}[Volume of neutral space]
% For a model defined in Definition \ref{def:para-func map}, 
% given dataset $S = (X, \mathbf{y}) \in \mathcal{X}\times\mathcal{Y}$
% and its neutral space $\mathcal{N}_S$ defined in Definition \ref{def:neutral space}
% , the volume of the specific neutral space 
% $\mathcal{N}_S$
% if defined as 
% \begin{equation}
%     V_{\mathcal{N}_S} = P(S) = P(\mathbf{y}\mid X) = 
%     \sum_{f} P(S \mid f) P(f)=\sum_{f \in \mathcal{C}_S} P(f) \\
%     = \int_{\theta \in \mathcal{N}_S} P(\theta) d\theta
% \end{equation}
% with $\mathcal{C}_S$ denoting the set of all functions compatible with the dataset
% $S$.
% \label{def:volume}
% \end{definition}
% By Definition \ref{def:volume}, although there can be infinite 
% parameter configurations in the neutral space
% (as we see in the ``re-scaling problem")
% , the volume of it, however, is well-defined and bounded.


